Cluster-to-adapt: Few Shot Domain Adaptation for Semantic Segmentation across Disjoint Labels

Domain adaptation for semantic segmentation across datasets consisting of the same categories has seen several recent successes. However, a more general scenario is when the source and target datasets correspond to non-overlapping label spaces. For example, categories in segmentation datasets change vastly depending on the type of environment or application, yet share many valuable semantic relations. Existing approaches based on feature alignment or discrepancy minimization do not take such category shift into account. In this work, we present Cluster-to-Adapt (C2A), a computationally efficient clustering-based approach for domain adaptation across segmentation datasets with completely different, but possibly related categories. We show that such a clustering objective enforced in a transformed feature space serves to automatically select categories across source and target domains that can be aligned for improving the target performance, while preventing negative transfer for unrelated categories. We demonstrate the effectiveness of our approach through experiments on the challenging problem of outdoor to indoor adaptation for semantic segmentation in few-shot as well as zero-shot settings, with consistent improvements in performance over existing approaches and baselines in all cases.

==> eccv2020kit/scripts/Introduction.tex <==
\section{Introduction} 

% Recent improvements in many computer vision tasks can be attributed to the progress of deep learning coupled with availability of large corpora of data and computational resources. 
In this work, we address the problem of knowledge transfer across domains with disjoint labels for semantic segmentation.
In spite of massive strides in computer vision performance using deep learning~\cite{lecun2015deep}, models trained on a large-scale labeled dataset are not guaranteed to generalize to data that lies outside the training distribution.
%
% training models that achieve state of the art performance on many tasks.
% However, , while obtaining large scale labeled data in every target domain is restrictive, expensive or simply not feasible due to many practical and social implications. 
%
% This phenomenon of dataset bias~\cite{torralba2011unbiased,tommasi2017deeper} is observed mainly because deep networks tend to learn many domain specific properties during training that adversely affect its generalizability. 
This difficulty is amplified for applications like semantic segmentation, where collecting pixel level labeled data for all geographies, environments and weather conditions is restrictive, expensive or simply not feasible due to many practical and social implications~\cite{kalluri2019universal}. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{eccv2020kit/scripts/figures/dataset_distances-NeuRIPS_al_fig.pdf}
    \captionsetup{width=0.5\textwidth}
    \caption{We illustrate the major challenge in our setting arising due to negative transfer. In our setting where source and target do not contain shared label space, traditional adversarial methods relying on global adaptation might lead to unrelated classes aligning with each other. In contrast, our method encourages only related classes to align with each other (selective alignment), while preventing negative transfer among unrelated classes.}
    \label{fig:illustration}
\end{figure}
  
  
% As a result, there has been considerable push towards learning domain invariant and transferable feature representations using limited labeled data. 
%
Unsupervised domain adaptation emerged as a feasible alternative to transfer knowledge from a labeled source domain to unlabeled target domains by minimizing some notion of divergence between the domains~\cite{long2017deep,long2015learning,sun2016deep,ganin2016domain,tzeng2017adversarial,bousmalis2016domain}.
% Previous works use divergence metrics based on MMD~\cite{long2017deep,long2015learning}, correlation alignment~\cite{sun2016deep} or adversarial feature alignment~\cite{ganin2016domain,tzeng2017adversarial,bousmalis2016domain} to learn domain agnostic representations. 
Prior works in domain adaptation are based on a global distribution alignment objective, assuming that the source and target datasets share the same label space so that domain alignment would invariably result in learning transferable feature representations. 
\input{eccv2020kit/scripts/intro_figure}
% However, this assumption rarely holds in real world and a more general setting is when the source and target datasets have different categories. 
% Previous works such as open set adaptation and partial adaptation~\cite{saito2018open,cao2018partial} relax this assumption to some extent by assuming only partial overlap between the source and target labels and reject unknown classes that fall outside the overlap. 
%
% Unlike these approaches, we propose a generic adaptation framework for a more general and useful setting with non-intersecting source and target label spaces. 

In many cases, the source and target labels might be completely distinct and share only high level geometric and semantic relationships. This makes it hard, yet necessary in few-shot settings, to perform useful knowledge transfer. In particular we show this in case of adaptation between outdoor datasets, where synthetic datasets are readily available, and indoor scenes, where we have few labeled data and it is considered difficult to render or maintain synthetic datasets. 
To address this challenging setting of outdoor to indoor adaptation, we propose a novel framework for adaptation across disjoint labels. For disjoint labels, we posit that a more suitable objective is to achieve \textit{domain invariance} with respect to related categories and \textit{domain equivariance} with respect to unrelated categories between source and target, thus avoiding negative transfer.
For example, the categories that frequently occur in an indoor environment like wall, floor, ceiling and chair are completely distinct from any outdoor categories, yet we show how we can leverage useful discriminative information through implicit geometric and semantic correspondences.

%
% As an example for semantic segmentation, the categories that frequently occur in an indoor environment like wall, floor, ceiling and chair are completely distinct from any outdoor categories, yet we can leverage useful discriminative information from labels like building, road, sky etc. 
% Even if a complete one-to-one mapping is not possible, a small subset of source labels might share properties with another subset of target labels. Models trained with such an objective  should achieve . Classical adversarial or global alignment based adaptation approaches would not address such category specific alignment resulting in potential negative transfer. 

In practice, the distribution shift between such source and target domains arise from both low-level (lighting, contrast, object density etc.) and high-level (category, geometric orientation, pose etc.) variations~\cite{bousmalis2016domain}. To ease this extreme case of adaptation, we introduce an additional unlabeled auxiliary domain, which shares properties with both the source and target datasets and would act as a bridge to improve the adaptation. 
For instance, adaptation from synthetic outdoor to real indoor datasets can benefit from unlabeled images from real outdoor scenes, as explained in~\figref{fig:dataset_relation}.  


To automatically discover related and unrelated categories across datasets, we propose a novel clustering based alignment approach called Cluster-to-adapt (C2A). C2A stems from the intuition that related categories from source and target should lie close to each other in the feature space for effective knowledge transfer. We realize this during training through a deep constrained clustering framework by posing the alignment as a clustering objective in a transformed feature space, which would force related categories to group close to each other while leaving room for unrelated categories to form independent clusters, as shown in~\figref{fig:illustration}.

% In summary, we make the following contributions.
% \vspace{-1em}

% \begin{tight_itemize}
%     \item A novel cluster-to-adapt (C2A) approach is proposed to effectively perform category level adaptation between semantic segmentation datasets with disjoint labels, using an intermediate domain with shared properties.
%     % \item We address the most general domain adaptation setting of knowledge transfer across datasets with completely distinct label spaces for semantic segmentation.
%     \item We make use of a computationally efficient clustering framework that helps in reducing the distance between related categories across datasets during training while preventing negative alignment between unrelated categories.
%     \item We demonstrate through empirical results that our proposed C2A approach consistently outperforms related approaches and baselines in fewshot as well as zeroshot settings for adaptation between outdoor and indoor segmentation datasets.
% \end{tight_itemize}





==> eccv2020kit/scripts/ProblemDescription.tex <==
\section{Framework}

We now explain our proposed approach, which addresses the most general case of knowledge transfer between domains with different, and non-overlapping label spaces. 
%
Denote using $\D_s$ the completely labeled source domain data with label space $\Y_s$, where $\D^s \sim p_s$(source distribution). The labeled target domain data is denoted by $\D_t$, with label space $\Y_t (\neq \Y_s)$, and $\D_t \sim p_t$(target distribution).
% , so they are essentially different tasks following the nomenclature in~\cite{pan2009survey}. 
We assume that a small subset $\D_t^l$ of the target data is labeled, for learning some task specific information like classifier boundaries, and the rest $\D_t^u$ as unlabeled, making our setting that of \emph{few-shot adaptation across domains with disjoint labels}. We denote this small fraction of labeled samples by $\sigma = |\D_t^l|/(|\D_t^u| + |\D_t^l|)$. Following the nomenclature of \cite{pan2009survey}, we henceforth call this as cross-task adaptation and the source and target as different tasks. In section \ref{sec:experiments}, we show results varying $\sigma$ from $0.01$ to $0.3$.
% We are mainly interested in cases when $ \sigma \ll 1 $.
In our case, the domain gap between the target data and source data comes from two factors, namely domain shift due to $p_s \neq p_t$ as well as label shift due to $\Y_s \neq \Y_t$. Furthermore, we do not assume any partial overlap between the label spaces unlike other partial or open set adaptation approaches which makes our setting more challenging. To ease the adaptation process across these widely different datasets, we introduce another completely unlabeled auxiliary domain $\D_a$, which serves as a useful bridge between the source and target datasets. For example, $\D_a$ could share \textit{task/content} properties with $\D_s$ and \textit{style} properties with $\D_t$. We show how to best exploit this completely unlabeled intermediate domain to achieve our primary goal of learning transferable features from source to target.
%
% Similarly, $\U_1=\{X_i^t\}$ is the unlabeled target domain data for task $\T_i$ task where $X_i^t \sim q_i$. For any particular task $\T_i$, $p_i \neq q_i$ and we refer to this as the \textit{within task domain gap}. Since $\Y_i \neq \Y_j$ for any $i \neq j$, $\T_i$ and $\T_j$ are essentially different tasks following the nomenclature in~\cite{pan2009survey}. Also, $q_i \neq q_j$ for any $i \neq j$, and we refer to this as the \textit{cross task domain gap}. We instantiate our approach for $n=2$ tasks in the rest of the paper for ease of demonstration while noting that the approach can be easily scalable to jointly train any number of tasks. 
% Clearly, addressing the latter is more challenging than addressing the within task domain gap.

\input{eccv2020kit/scripts/arch_fig}

\noindent {\bf Overview} We present the overview of the proposed network architecture in~\figref{fig:main_schematic}. We use a shared encoder $\E:(H,W,3) \rightarrow (H',W',f_d)$ across all the datasets which aggregates spatial features across multiple resolutions of the input image $x$, and outputs a downsampled encoder map $\E(x)$. $f_d$ is the size of features in the encoder map. Since shallow level features are known to be more task agnostic and transferable~\cite{yosinski2014transferable}, a shared encoder helps us to learn generic features useful across source and target datasets. Task specific decoders $\Dec_s$ and $\Dec_t$ then upsample the output of the encoder and compute class assignment probabilities for each pixel of the input image over the label space $\Y_s$ and $\Y_t$ respectively. Individual decoders for source and target helps us to make predictions over respective label spaces. The supervised loss computed using the labeled data from source and target datasets is given by  
\begin{equation}
    \Loss_{sup} = \Loss_{sup}(\D_s) + \Loss_{sup}(\D_t^l),
    \label{eq:supervised_loss}
\end{equation}
where
\begin{IEEEeqnarray}{rCl}
    \Loss_{sup}(\D_s) &=& \frac{1}{N_s} \nonumber \\ &&\sum_{\substack{(x,y) \in \{\D_s\}}} \frac{-1}{H W} \sum_{h,w} \log(\Dec_s(\E(x))^y(h,w))) \IEEEeqnarraynumspace
\end{IEEEeqnarray}
and $N_s$ is the number of labeled samples in the source dataset, and $H,W$ are the height and width of the output feature map respectively. The target supervised loss $\Loss_{sup}(\D_t^l)$ is defined similarly.  
% We then calculate the supervised loss $\Loss_{sup}$ using these predictions and the ground truths available from source data.  

% However, training $\E$ and $\Dec$ on labeled source data alone would not perform well on target data due to \textit{within task domain gap}. 
% To address the within-task domain gap challenge, 
%
Next, we decouple the source to target alignment into two different objectives. The first is a \textit{within task} alignment between $\D_s$ and $\D_a$, and the second is the \textit{cross task alignment} objective between $\D_a$ and $\D_t$, as explained next. 
% This successive adaptation approach performs better than direct adaptation between source to target by making use of the intermediate bridging domain.
% 
% We also found that presenting $\Prob_i(x)$ stabilizes the training as it disentangles the within task alignment objective
%
% Although training with task specific discriminators performs much better than naive joint training with source datasets,
%
% However, training $\E$ and $\Dec$ with task specific supervised loss and adversarial alignment losses alone would not perform well due to cross-task domain gap, since we do explicitly transfer any semantic relations among the tasks.
%
% To perform \textit{within task} alignment, we use an adversarial alignment objective, under the assumption that the domain shift between $\D_s$ and $\D_a$ arise from low-level differences only, and the label spaces are shared. Similar adversarial constraint cannot be imposed for adaptation between $\D_a$ and $\D_t$ due to both low level and high level differences. To handle this challenging \textit{cross task alignment} objective, we introduce a feature transformation layer $\FTN$.
% which takes the output of the encoder as input and projects it into a lower dimensional subspace suitable for a clustering objective. Combining these modules during training, our total objective function consists of a supervised loss term $\Loss_{sup}$, an adversarial alignment objective $\Loss_{adv}$ as well as a constrained clustering based cross task alignment objective $\Loss{c}$. 
%
% output as the input maps the $(H',W',f)$ size encoder map into a lower dimensional subspace $(H',W',f_t)$. 

% \subsection{Supervised Loss} 
% The supervised loss is computed using the labeled data from source and target datasets. For every labeled input image from $\D_s$ and $\D_t$, we compute the pixel wise cross entropy loss over the number of classes from that dataset. The final loss is the total cross entropy loss from the source and target datasets given by
% \begin{equation}
%     \Loss_{sup} = \Loss_{sup}(\D_s) + \Loss_{sup}(\D_t^l),
%     \label{eq:supervised_loss}
% \end{equation}
% where
% \begin{equation}
%     \Loss_{sup}(\D_s) = \frac{1}{N_s} \sum_{\substack{(x,y) \in \{\D_s\}}} \frac{1}{H \cdot W} \sum_{h,w} - \log(\Dec_s(\E(x))^y(h,w)))
% \end{equation}
% and $N_s$ is the number of labeled samples in the source dataset, and $H,W$ are the height and width of the output feature map respectively. The target supervised loss $\Loss_{sup}(\D_t^l)$ is defined similarly.  

\subsection{Within Task Domain Alignment}

We introduce the within task alignment objective between the source and intermediate domains $\D_s$ and $\D_a$. We assume that the domains share the same label space and exhibit only low-level differences, and use an adversarial alignment strategy using a domain discriminator $\Disc$. 
% Specifically, we train a discriminator $\Disc$ to differentiate the outputs from the source and auxiliary datasets, and simultaneously train the generator which produces representations that are indistinguishable from each other.  
% Training $\E$ and $\Dec_i$ on labeled source data alone would not perform well on target data which is of real interest. In our case, this happens because the marginal distributions of the source and target data within a task $\T_i$ are different. We refer to this as the within task domain gap. 

Following the idea presented in~\cite{tsai2018learning}, we send the output probability maps $\Prob_s(x) = \Dec_s(\E(x))$ to the discriminator $\Disc$ as opposed to the encoder maps. This helps in better within-task alignment for pixel level prediction tasks and, as we found out, faster convergence during training. We train the discriminator $\Disc:(H,W,|\Y_s|) \rightarrow \{0,1\}$ which takes as input the output map of the generator, to output the probability of the map coming from source data. The generator is then trained to produce outputs from $\D_a$ which are good enough to trick the discriminator into classifying them as coming from source. This alternative min-max optimization would then result in domain invariant output maps leading to successful feature alignment. 
% We also found that LS-GAN~\cite{mao2017least} which uses a least-squares objective worked better than a Vanilla GAN which uses a binary cross entropy objective~\cite{goodfellow2014generative}. 
% so that the source classifier can be directly transferred to the target examples. 
%
The adversarial loss, using LS-GAN~\cite{mao2017least}, is given by
\begin{equation}
    \Loss_{adv} = \mathrm{E}_{x \sim \D_a} (\Disc(\Prob_s(x)))^2 
\end{equation}
and the discriminator objective $\Loss_D$ is given by 
\begin{equation}
    \Loss_{\Disc} = \mathrm{E}_{x \sim \D_s} (\Disc(\Prob_s(x)))^2 + \mathrm{E}_{x \sim \D_a} (\Disc(\Prob_s(x))-1)^2
\end{equation}

Although we use this adversarial adaptation strategy for within-task alignment, we note that our method can also be applied in combination with any other adaptation strategy based on generative modeling or distribution matching~\cite{murez2018image,yang2020fda,vu2019advent} for within task alignment.
% More importantly, our goal in this paper is not to improve the performance on within task domain alignment, but rather to propose an effective way to transfer semantic relations between datasets with different categories in an unsupervised fashion, which we present next.

% We observed that using a single common discriminator across all the tasks would make it very easy to distinguish source samples from target making the discriminator's job easier. This is because the domain gap between a source and target from two different tasks is much larger than source and target from the same task. Hence it is necessary to use individual task-specific discriminators. 

% as the complete global distribution alignment of all the source and target representations might induce some negative alignment across tasks as they might not necessarily share the same label space. It might often also be the case that some features can be aligned across tasks for better semantic transfer~\cite{luo2017label}. To handle this case, 

\subsection{Cross Task Semantic Transfer}
% \vspace{-.5em}

Training $\E$ and $\Dec$ with task specific supervised loss and adversarial alignment losses alone is insufficient to transfer useful semantic content to target dataset, since we do not explicitly transfer any semantic relations between the tasks. Naive adversarial training of yet another discriminator to distinguish outputs from two tasks would not work well, as we only want categories that share semantic cues to align with each other (selective alignment) as opposed to global alignment (\figref{fig:illustration}). Luo et. al.~\cite{luo2017label} propose using an entropy minimization objective after computing pairwise similarity of the features, but computing such pairwise similarity is computationally infeasible for pixel level prediction tasks.
%
Towards this goal, we propose a novel deep clustering based approach, which lies at the core of our approach.

\paragraph{\emph{\textbf{Constrained Clustering Objective}}}
% Distance metric. 
Following the assumption that deep features form discriminative clusters in the feature space useful for classification tasks~\cite{chapelle2005semi}, we believe that better knowledge transfer would happen across tasks if the features of categories which share semantic information also form coherent clusters closer to each other. A major challenge with incorporating this constraint in deep neural networks is the lack of information regarding the correspondence between categories of the datasets useful in preventing negative transfer effects. 
% In the most challenging setting, the label spaces might be completely distinct i.e, $\Y_s \neq \Y_t$, so universal adaptation methods~\cite{you2019universal} are not suitable.
We use a clustering based objective to discover the similarity across categories, and enforce the clustering constraint by performing k-means clustering of the feature vectors. This encourages the features corresponding to similar categories across tasks to form a single ``meta-cluster", while leaving room for unrelated categories to form independent clusters.  

We first pass the outputs of the shared encoder $\E$ through a feature transfer module $\FTN:(H',W',f_d) \rightarrow (H',W',f_e)$, where $f_e$ is the feature dimension in the transformed space. $\FTN$ is necessary because the features learnt specific to a task might not be suitable for cross-task semantic transfer directly in the feature space. A learnable transformation function would, instead, find the best subspace amenable for alignment. Also, since $f_e \ll f_d$, the feature transformation would result in efficient computation of centers and similarity metrics for k-means. We formulate our constrained clustering objective using the cross-entropy loss, given by 
\begin{equation}
    \Loss_c = \sum_{x \in  \{\D_a , \D_t^u\}} \sum_{v_j \in \FTN(\E(x))} - \log (\max_k p(\mu_k | v_j))
    \label{eq:clustering_loss}
\end{equation}

\noindent where $p(\mu_k|v_j)$ is the probability score that a feature vector $v_j$ belongs to a cluster with center $\mu_k$, and
\begin{equation}
    p(\mu_k | v_j) \propto \exp \left( \frac{v_j \cdot \mu_k}{||v_j||_2 ||\mu_k||_2} \right)
\end{equation}

% \noindent The choice of (normalized) cosine function as a similarity metric is empirically motivated, as we find this objective to perform better in our setting than the euclidean distance based similarity function.

% \paragraph{\emph{\textbf{Feature Transformation Layer}} }
% We use a feature transformation layer $\F$, 
% The outputs of the shared encoder $\E$ are first transformed to another lower dimensional subspace~\figref{fig:schematic} using a feature transfer module $\FTN:(H',W',f_d) \rightarrow (H',W',f_e)$, where $f_e$ is the feature dimension in the transformed space, and we choose $f_e < f_d$.

% \noindent Directly applying \eqref{eq:clustering_loss} over features from the output of the encoder  

% Practically, we found that the following helps. 


\paragraph{\emph{\textbf{Avoiding Trivial Solution}}} Direct optimization of~\eqref{eq:clustering_loss} would quickly lead to a trivial solution where all the vectors are mapped to a single cluster.
% , which is a common phenomenon with many deep clustering based approaches~\cite{caron2018deep,zhang2019framework}. 
We found that initializing the cluster centers using features computed from pretrained network on labeled target data alone ($ \D_t^l$, trained offline) would reduce this problem to a large extent. 
% Details on initializing and efficiently updating the clusters can be found in the supplementary material.
%
% Supplementary: Explain in detail how to come up with initial set of centers
%
Additionally, we follow the idea proposed in~\cite{xie2016unsupervised}, and add a self-training constraint which encourages uniformity among the clusters and the cluster assignment probabilities are forced to be equal to an auxiliary target distribution. Specifically, we would like to have the target distribution $q(\mu_k | v_j)$ to hold the property that 
\begin{equation}
    q(\mu_k | v_j) \propto p(\mu_k | v_j) \cdot p(v_j | \mu_k)  \nonumber
\end{equation}

\noindent The first term on the RHS would improve the association of correct points to clusters, while the second term would discourage very large clusters. Applying bayes rule would give us the form of the target distribution as
\begin{equation}
    q(\mu_k | v_j) = \frac {{ p(\mu_k | v_j)^2}/ {\sum_j p(\mu_k | v_j)} } { \sum_{k'} { p( \mu_{k'} | v_j)^2} /{\sum_j p( \mu_{k'} | v_j)}   }.
\end{equation}

\noindent The constraint is now enforced in the form of a KL-Loss between the source distribution and the auxiliary target distribution. 
\begin{IEEEeqnarray}{rClCl}
    \Loss_{kl} &=& KL(p||q) \nonumber \\ &=& \sum_j \sum_k q(\mu_k | v_j) \log \left(\frac{q(\mu_k | v_j)}{p(\mu_k | v_j)} \right)
    \IEEEeqnarraynumspace
\end{IEEEeqnarray}

% \vspace{-1em}
\noindent The final training objective for the model can be summarised as follows,
\begin{eqnarray}
    \argmin_{\E,\Dec_s,\Dec_t,\FTN} & \,\,\, \Loss_{sup} + \lambda_{adv} \Loss_{adv} + \lambda_{c} (\Loss_{c} + \Loss_{kl}) \nonumber \\
    \argmin_{\Disc} & \Loss_{\Disc} 
\end{eqnarray}

\vspace{-1em}
\noindent where $\lambda_{adv}$ and $\lambda_c$ are the coefficients which control the relative importance of the adversarial loss and clustering loss respectively. The optimization is done by alternating between the two objectives within every iteration. A crucial factor in our method is the initialization of cluster centers before training, and we discuss our strategy followed for it next.

\subsection{Cluster Initialization}

The cluster centers are initialized using networks pretrained on the limited labeled data. Specifically, we use the same architecture as described in the paper to train a model on the labeled source data $\D_s$ as well as sparsely labeled target data $\D_t^l$ using pixel level cross entropy loss. We then pass the unlabeled images from the target $\D_t^u$ and collect all the encoder maps corresponding to all the images. Each encoder map is of size $(H/8 , W/8 , 2048)$ for our ResNet-101 backbone. To match the dimension of the FTN output, which is $128$ in our case, we apply PCA over these feature vectors to reduce their dimension. Then, a clustering is performed using the classical k-means objective with $K$ cluster centers, and the resulting centers are used to initialize $\mu_k's$ in the downstream adaptation approach. 

\paragraph{ \emph{\textbf{Efficient Computation of Centers}}} In traditional k-means, the centers $\mu_k$ are calculated using an iterative algorithm consisting of cluster assignment and centroid computation repeated until convergence. We mention a couple of issues persistent with this approach. Firstly, for dense prediction tasks like semantic segmentation, the encoder map consists multiple feature vectors which correspond to different patches of the input image. For example, an encoder map of size $(H',W')$ has $H' W'$ vectors of size $f_e$. Performing k-means over these vectors collected over all images over all the tasks would demand huge storage and computation requirements. Secondly, switching between gradient based training of network parameters and iterative computation of cluster centers after every few iterations would lead to an inefficient procedure that is not end-to-end trainable. To counter these limitations, we follow the idea proposed in ~\cite{han2019learning} and include $\mu_k$ as trainable parameters in the network, and update them after each iteration based on the gradients received from $\Loss_C$. 

% It is still remains to identify the ideal number of clusters, $K$, suitable for the task. The number depends on the problem at hand and the degree of relationship between categories across the different tasks. 
% Choosing a very small value for $K$ would give rise to many noisy alignments, and a very high value would not result in the semantic alignment we are after. 
% As we show in \secref{subsec:experiment_on_clusters}, we empirically determine $K=10$ clusters to suit the best for our task. 

==> eccv2020kit/scripts/Relatedwork.tex <==
\section{Related Work}

% Our work is closely related to works in domain adaptation for semantic segmentation and deep clustering, which are compared and contrasted below.

% \vspace{-.5em}
% In this section, we review some related literature.
% some works in literature which are related to our approach. 

% \paragraph{\textbf{Semantic Segmentation}}
% Semantic segmentation corresponds to pixel level classification of an image into predefined categories. Recent progress in deep learning~\cite{lecun2015deep,krizhevsky2012imagenet} has greatly benefited the progress in semantic segmentation, through architectures which use a combination of fully convolutional networks~\cite{long2015fully,badrinarayanan2017segnet}, dilated convolutions~\cite{yu2017dilated} and multi-scale estimations~\cite{chen2017deeplab} achieving state of the art performance with near real-time inference~\cite{romera2017erfnet,sandler2018mobilenetv2}, when trained on large scale labeled data such as Cityscapes~\cite{cordts2016cityscapes} or IDD~\cite{varma2019idd} for outdoor scenes and SUNRGB~\cite{song2015sun} for indoor scenes. 

% % . Long et. al.~\cite{} introduce a fully convolutional architecture in which segmentation is performed by aggregating predictions across multiple scales of the output map. Following this, many frameworks based on the encoder-decoder model have been proposed in literature \cite{,,ronneberger2015u,,} which have since widely improved state of the art performance on semantic segmentation. 
% % Frameworks that offer efficient inference ~\cite{romera2017erfnet,sandler2018mobilenetv2} offer segmentation models with efficient inference times. 
% %
% To avoid this contingency on the availability of large scale datasets in every domain which might not be always available, we propose a way to transfer knowledge from already existing large scale segmentation datasets, such as outdoor driving scenes to completely novel target domains, such as indoor scenes.

% However, the superior performance of these architectures is heavily contingent upon  with pixel level labels like . Such large scale labeled data , and it is essential to train segmentation models that perform well universally~\cite{kalluri2019universal} across data rich as well as data poor domains. Therefore, .
% The models trained models often end up learning representations very specific to a dataset with poor generalization possibilities to data that lies outside this distribution.
%
% As a step towards mitigating this unwanted property, in this work, we introduce an efficient approach to learn generic representations that are useful across diverse tasks, like indoor and outdoor segmentation, 
% without using any external knowledge graph like~\cite{liang2018dynamic} or target supervision like~\cite{kalluri2019universal}.
% with minimum labeling overhead.

% Synthetic datasets~\cite{} emerged as a viable alternative, but models trained on synthetic datasets do not generalize well to real datasets or new tasks. In this work, we propose a simple yet efficient way to transfer useful knowledge 

% Huge overhead for labeling and annotating datasets. Suffer from domain gap - do not transfer well. We feel that there is a need to learn generic data representations completely from unlabeled data. 

% \paragraph{\textbf{Universal Representation Learning}} 

% Multi task learning have been very popular and relevant. Universal prediction is a type of multi-task learning setup where a single model is trained to perform different tasks from different datasets with different distributions. Reduce the deployment cost. Learning multiple tasks from single image/data. More challenging is the case when need to use single model to perform completely different tasks on diverse domains. Needs adaptation with limited labeled data. 

\paragraph{\textbf{Unsupervised Domain Adaptation (UDA)}}

% Deep learning models trained on a source domain do not generalize well to target data outside the source distribution due to a phenomenon called dataset bias~\cite{torralba2011unbiased}.
% This problem is amplified in deep neural networks as the representations learnt by the deeper layers are often domain specific~\cite{yosinski2014transferable}. 
UDA is used to transfer knowledge from a large labeled source domain to an unlabeled target domain. Large body of works that perform adaptation from labeled source to unlabeled target rely on adversarial generative~\cite{bousmalis2017unsupervised,sankaranarayanan2018generate,murez2018image,hoffman2017cycada, zou2019confidence} or  discriminative~\cite{ganin2016domain,tzeng2017adversarial,tzeng2015simultaneous,hoffman2016fcns} approaches to learn domain agnostic feature representations. 
% Other works also explore centroid alignment~\cite{pan2019transferrable,xie2018learning,pinheiro2018unsupervised} for feature adaptation. 
% Centroid alignmentcentroid alignment~\cite{} approaches.
% Numerous appraoches exists towards unsupervised domain adaptation, and we summarize few works which use adversarial approaches here.
%
% While Ganin et. al. introduce a gradient reversal layer in~\cite{ganin2016domain}, authors in \cite{tzeng2017adversarial,tzeng2015simultaneous,tsai2018learning} use GAN loss to fool a discriminator trained to classify the source and target domains, thereby learning domain invariant features. Adversarial generative methods have been explored in~\cite{} to translate images between source and target domains for domain adaptation, and recent works also propose ,  tri-training~\cite{saito2017asymmetric} or self-ensembling~\cite{shu2018dirt,french2017self} as effective methods to perform feature alignment between source and target distributions.
%
A common assumption in most of these approaches is that the source and target label spaces completely overlap, so that a classifier learnt on the source domain can be directly applied on the target data. However, in most real world applications this assumption is invalid, and in most general case, the categories might be completely different. Very few works exist which address this more challenging setting.
% In extreme contrast, it might be useful to transfer knowledge even between datasets  with completely non-intersecting label spaces. 
Previous works like open set adaptation~\cite{saito2018open}, partial set adaptation~\cite{cao2018partial,cao2019learning} and universal adaptation~\cite{you2019universal, kalluri2019universal} assume some degree of label overlap, \cite{luo2017label} performs adaptation between distinct label spaces with few target labeled data using pairwise similarity constraints, while \cite{sohn2018unsupervised} addresses adaptation for verification tasks which is different from our focus on semantic segmentation. Similarly, more recent works for domain adaptation suited for semantic segmentation tasks \cite{lv2020cross, musto2020semantically, yang2020fda, mei2020instance, wang2020classes, araslanov2021self} achieve state of the art results for the case of completely overlapping label spaces in the source and target domains, and are not applicable in our setting of outdoor to indoor adaptation.
In contrast to these existing works, we propose an efficient method to align only visually similar features across source and target domains which can have completely non-intersecting label spaces without re-annotation~\cite{lambert2020mseg}, while preventing potential negative transfer, specifically suited to cross domain semantic segmentation.
% 

\paragraph{\textbf{Deep Clustering}} Although clustering algorithms like k-means~\cite{macqueen1967some} are extremely useful in automatically discovering structure from unlabeled data~\cite{aggarwal2014data}, they work directly on the high dimensional input space like images which is often ineffective for classification. Recent works propose jointly learning a suitable feature representation of data along with clustering assignments. For example, \cite{hsu2017learning} uses pairwise similarity based constraints, while~\cite{han2019learning} uses self-training objective on the cluster assignment scores to successfully perform unsupervised transfer across categories from the same domain. Other works make use of deep clustering to learn more discriminative clusters~\cite{xie2016unsupervised} useful for classification, or as suitable pretext tasks in self supervised learning~\cite{caron2018deep,caron2019unsupervised,yan2019clusterfit}. While deep clustering based approaches have been previously applied in the case of unsupervised category discovery~\cite{han2019learning}, we extend this idea to additionally account for the domain shift between the source and target datasets.
% We extend the ideas proposed in deep clustering literature to perform unsupervised cross task adaptation.
% , using a novel constrained clustering algorithm in a transformed feature space. 
% without any similarity constraints like ~\cite{hsu2017learning}
% To avoid  clustering is a related paradigm where the cluster assignments are constrained to obey certain properties like pairwise similarity ~\cite{hsu2015neural}
%

\textcolor{black}{Also, note that many prior works that use clustering for adaptation consider the classical setting of completely matching source and target domains \cite{DBLP:conf/wacv/ToldoMZ21, DBLP:conf/eccv/WuHLUGLD18, DBLP:journals/corr/abs-2012-04280} or partial overlap in open world setting \cite{DBLP:conf/cvpr/GongCPLCLDG21}, and hence use clustering as a means to achieve one-to-one alignment between source and target. In contrast, we use clustering to selectively align source and target across completely disjoint label spaces. }



% works for unsupervised task transfer. we use it for selective visual feature alignment across features from different tasks in addition to the adversarial losses.





==> eccv2020kit/scripts/abstract.tex <==


\begin{abstract}
%
Domain adaptation for semantic segmentation across datasets consisting of the same categories has seen several recent successes. However, a more general scenario is when the source and target datasets correspond to non-overlapping label spaces. For example, categories in segmentation datasets change vastly depending on the type of environment or application, yet share many valuable semantic relations. Existing approaches based on feature alignment or discrepancy minimization do not take such category shift into account. 
In this work, we present Cluster-to-Adapt (C2A), a computationally efficient clustering-based approach for domain adaptation across segmentation datasets with completely different, but possibly related categories. 
We show that such a clustering objective enforced in a transformed feature space serves to automatically select categories across source and target domains that can be aligned for improving the target performance, while preventing negative transfer for unrelated categories. 
We demonstrate the effectiveness of our approach through experiments on the challenging problem of outdoor to indoor adaptation for semantic segmentation in few-shot as well as zero-shot settings, with consistent improvements in performance over existing approaches and baselines in all cases. 
% Code and models will be publicly released. 
% We also validate our approach on a novel zeroshot adaptation setting 
%
% Although deep neural network models trained on large amounts of labeled data perform exceedingly well, the performance drops significantly when deployed on unseen datasets. In this context, domain adaptation is greatly useful in learning representations from a large source domain that are transferable and generalize well to novel target domains. However, it is often not feasible to assume that large labeled source data would always be available, so it is essential to learn 
% However, it is still an open problem to transfer learned representations across tasks with different label spaces, especially for problems like semantic segmentation where the label spaces change vastly depending on the type of dataset. 
%
% Global distribution alignment between the features from two tasks is not possible, so we propose a novel constrained clustering algorithm which is useful in aligning only visually similar features across different tasks. 
%
%
% datasets and achieve competitive results compared to existing baselines in addition.   
%
%% Domain adaptation is useful.
%% Cross task adaptation is relatively less explored. Often availability of large labeled data in a source domain of same task is invalid. 
% We introduce a cross task adaptation approach for semantic segmentation - using labeled data from an entirely different task. We perform. To further alleviate the domain gap, we introduce an auxiliary bridge domain that further serves to reduce the gap between the two domains. 

% \keywords{Semantic Segmentation, Domain Adaptation, \\Transfer Learning}

\end{abstract}

==> eccv2020kit/scripts/conclusion.tex <==
 \vspace{-8pt}
\section{Conclusion}
% \vspace{-1em}

% Though this work, we tackle the extremely challenging problem of . 
% In spite of being the most general setting for knowledge transfer, adaptation between domains with non-overlapping label spaces is largely understudied. 
We introduce C2A, a clustering based approach called C2A to study the most general, yet largely understudied setting of adaptation between domains with non-overlapping label spaces for feature alignment across source and target datasets with disjoint labels. C2A encourages positive alignment of visually similar feature representations while preventing negative transfer. We experimentally verify the effectiveness of our approach on the task of outdoor to indoor adaptation for semantic segmentation and demonstrate significant improvements over existing approaches and prevalent baselines in both fewshot and zeroshot adaptation settings. 
% We hope that our work encourages the community to collect generic datasets useful for universal adaptation for semantic segmentation.
% In future, we aim to develop the idea of selective feature alignment using metric based loss functions.
% Conclude your paper. In future, we might want to investigate further into various other recently proposed methods for task transfer learning for tackling fundamentally different tasks like detection and classification. We can also look at other cluster constraints in terms of similarity, global size constraint etc. 

==> eccv2020kit/scripts/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\input{eccv2020kit/scripts/table_results}

% We now validate the effectiveness of the proposed approach using empirical results on a challenging setting of adapting outdoor synthetic datasets like GTA~\cite{richter2016playing} and Synthia~\cite{ros2016synthia} to indoor real datasets like SunRGB~\cite{song2015sun}, using Cityscapes~\cite{cordts2016cityscapes} as the unlabeled intermediate domain. 
% We present more details regarding the choice of datasets, the network architecture, training details and metrics in the supplementary section. 
% We present details regarding the choice of datasets, the network architecture, training details and evaluation metrics, followed by our experimental results. 
\subsection{Datasets} 

For the source dataset $\D_s$, we use synthetic images from the driving dataset GTA~\cite{richter2016playing}. GTA consists of 24966 images synthetically generated from a video game consisting of outdoor scenes with rich variety of variations in lighting and traffic scenes. We also show results using the SYNTHIA-RAND-CITYSCPAES split from Synthia~\cite{ros2016synthia} dataset, which consists of 9600 synthetic images with labels compatible with Cityscapes. 
For the target dataset $\D_t$, we use real images from SUN-RGBD~\cite{song2015sun} consisting of images from indoor scenes. SUN-RGBD consists of 5285 training images and 5050 validation images containing pixel level labels of objects which frequently occur in an indoor setting like chair, table, floor, windows etc. We use the 13 class version from~\cite{mccormac2017scenenet}. The background class is ignored during training and evaluation.
% We believe that this choice of datasets is significant because knowledge transfer between indoor and outdoor images for semantic segmentation was never explored in literature before. 
Additionally, we use the 2975 training images from Cityscapes~\cite{cordts2016cityscapes} dataset, which consists of outdoor traffic scenes captured from various cities in Europe, as the unlabeled auxiliary domain $\D_a$. Cityscapes shares its semantic categories with GTA, so that the variation between $\D_s$ and $\D_a$ is only due to synthetic and real appearance, while $\D_s$ and $\D_t$ have many low-level as well as high-level differences. 
% The semantic categories are shared between Cityscapes and GTA.

% Furthermore, we also test out approach in a complementary, yet related, setting of zero shot adaptation. Specifically, we assume that we do not have any labeled or unlabeled images from the target dataset. Instead, we assume we have access to synthetically generated images that share categories with the target dataset. To validate this approach, we use all the labeled images from SceneNet~\cite{mccormac2017scenenet} as the target dataset, and show the generalization capabilities to datasets not seen before.
% We report all our results on the validation set of SUN-RGBD datasets. 

\subsection{Training Details}
%
We use the DeepLab~\cite{chen2017deeplab} architecture with a resnet-101 backbone for the encoder framework $\E$. For the task-specific decoder $\Dec$, we use an ASPP convolution layer followed by an upsampling layer. The architecture of discriminator $\Disc$ is similar to DC-GAN~\cite{radford2015unsupervised} with four $4 \times 4$ convolution layers, each with stride 2 followed by a leaky ReLU non-linearity. The feature transformation module $\FTN$ is a $1 \times 1$ convolution layer with output channels equal to the embedding dimension, which is fixed as $f_e=128$ for all the experiments. We use a default value for $\lambda_{adv}=0.001$. Following~\cite{xie2018learning}, to suppress the noisy alignment during the initial iterations, we set $\lambda_c = \tfrac{2}{1+e^{-10*\delta}}-1$, where $\delta$ changes from 0 to 1 over the course of training. The backbone architecture is trained using SGD objective, with an initial learning rate of $2.5 \times 10^{-4}$. For training the cluster centers, we follow a similar learning rate decay schedule, but start with a smaller learning rate of $2.5 \times 10^{-5}$. This is because the cluster centers are already initialized using networks trained on the labeled data, and we would ideally like the centers to not drift too far away from their initial values.

% We use $\lambda_{adv} = \lambda_c = 1$.

\vspace{-1em}
% \subsection{}
\paragraph{\emph{\textbf{Baselines and Ablations}}}
We provide ablation studies of the clustering module proposed in our approach and compare with the existing baselines. Specifically, we provide comparisons against the following.
%
\begin{enumerate*}[label=(\roman*)]
  \item \textbf{Target Labeled Only}: We train the segmentation encoder and decoder using only the limited labeled data from the target domain, $\D_t^l$, 
  \item \textbf{Finetune}: We use a model trained on source dataset $\D_s$ till convergence, and finetune it on the labeled target data,
  \item \textbf{Ours (C2A), $\lambda_c=0$}: Our cluster to adapt approach, without the clustering objective, and
  \item \textbf{Ours (C2A)}: our proposed approach with all the losses included.
\end{enumerate*}

\vspace{-1em}
\paragraph{\emph{\textbf{Comparison with prior works}}} We reiterate the paucity of existing works which tackle the same setting as ours, making direct comparison hard. Many traditional adaptation methods prevalent in literature for segmentation~\cite{luo2019taking, hoffman2016fcns, sun2019not, vu2019advent} are not directly applicable in cases with disparate source and target label sets. Therefore, we compare against two competitive approaches that perform domain adaptation by extending them as follows.
% To provide comprehensive insights into the usefulness of our approach, we compare our work by extending a competitive approach that performs pixel level domain adaptation. 
\begin{enumerate*}[label=(\roman*)]
  \item \textbf{AdaptSegNet*}~\cite{tsai2018learning}: We choose \cite{tsai2018learning} as the backbone pixel level adaptation method for global adaptation across source and target datasets as it achieves high performance with a simple method. Since \cite{tsai2018learning} is not directly applicable to our case due to different labels spaces, we extend their method to perform feature space adaptation.
  \item \textbf{LET*}~\cite{luo2017label}: We compare against adaptation proposed in~\cite{luo2017label} using entropy minimization criterion. We extend it to suit the segmentation task by using class prototypes in the feature space instead of pairwise enumeration which keeps the computation feasible.
%   \item \textbf{Ours (C2A) , $\lambda_{adv} = 0$}: Our setting without using the intermediate domain $\D_a$.
\end{enumerate*}

\input{eccv2020kit/scripts/long_Classwise_table}

% \begin{wrapfigure}{r}{0.5\textwidth}
% %   \captionsetup{width=\textwidth}

% \end{wrapfigure}

\vspace{-1em}
\paragraph{\emph{\textbf{GTA to SunRGB}}} 
% In ~\tabref{tab:main_results}, we provide ablations with varying the amount of supervision from the 5285 images in the SUN-RGB training set. 
We show in \tabref{tab:main_results} our results by varying the amount of supervision by choosing $|\D_t^l| = \{50,200,500,1500\}$ images which corresponds to $\sigma = \{1\% , 4\% , 10\% , 30\%\}$ respectively. Our method based on a novel clustering objective consistently outperforms other approaches by considerable margins, more so in cases when there is extreme scarcity of labeled data. We see upto $~15\%$ and $~10\%$ relative increase in mIoU for $\sigma=1\%$ and $\sigma=4\%$ respectively compared to training only on the labeled target dataset. It is also evident that the clustering loss $\Loss_c$ is important for the objective to successfully carry selective alignments from source and intermediate domains to the target domain, as seen from improvements in our results compared to prior works like \cite{tsai2018learning} and \cite{luo2017label}. We also observed that 30\% is already sufficient data for supervised fine-tuning to do well without any adaptation. 
% Similar observations have been made for other semi-supervised adaptation works~\cite{zhang2018fully}. 
In this work, our goal is focused on boosting the adaptation performance when enough labeled examples are not present in the target domain ($\sigma \lll 1$). 

% Proposed approach also exhibits remarkably significant gains compared to state of the art segmentation models based on discriminative adversarial objective like AdaptSegNet~\cite{tsai2018learning}. This is because direct adversarial approach would perform global distribution alignment, which is not always suitable in settings where the categories from the datasets do not overlap. In contrast, our constrained clustering based approach would positively transfer discriminative information across only a set of selected distinct yet related categories.

\vspace{-.5em}
\noindent \paragraph{\emph{Role of intermediate bridge domain}}
The intuition behind using an intermediate domain is to ease the adaptation process between the synthetic source domain data and real target domain data, which differ in both the appearance and the label spaces (categories). 
The use of an unlabeled domain bridge leads to no degradation with respect to a direct GTA to SUN adaptation for N = 200 (33.5\% without and 33.4\% with), while leading to a noticeable benefit for N = 50 (25.0\% without and 26.0\% with bridge domain). 

\vspace{-.5em}
\noindent \paragraph{\emph{Comparison with semi-supervised learning methods}} We also compare our work with existing semi-supervised segmentation algorithms in literature, namely AdvSemiSeg~\cite{hung2018adversarial} and universal semi-supervised segmentation~\cite{kalluri2019universal} and include results in \tabref{tab:main_results}. For \cite{hung2018adversarial}, we use the unlabeled and labeled image sets from SUN-RGB to run the experiments. For \cite{kalluri2019universal}, we follow the setting of their paper and use N=(50,200,500,1500) labeled examples from source and target, and use rest of images without annotations. From table~\tabref{tab:main_results}, we note that our method delivers much better performance compared to semi-supervised learning methods for lower amounts of target supervision, as the latter do not leverage rich supervision available from a source domain.


\input{eccv2020kit/scripts/qualitative.tex}
\input{eccv2020kit/scripts/fig_and_table.tex}


\vspace{-.5em}
\noindent \paragraph{\emph{\textbf{Category-wise Performance}}} We show the classwise mIoU results of our method in \tabref{tab:class_wise_iou} for both cases of using GTA and Synthia as the source dataset. The proposed C2A approach outperforms the baselines, that do not make use of the alignment strategy, on most of the classes. The gains are especially significant on classes like floor, wall and ceiling, which share many geometric as well as semantic properties with categories in Cityscapes and GTA (\figref{fig:qualitative}). For example, the patches corresponding to road in GTA dataset can help to successfully identify the parts of indoor images that correspond to floor since both occur mostly in the lower parts of images and share many other appearance and geometric relations. 
% Similarly, in classes where there is no correspondence to any source category, the performance is retained showing absence of any negative alignment. This supports our initial hypothesis that knowledge transfer across different yet related classes would positively affect the overall performance in cases when target labeled data is very low.

\vspace{-1em}
\noindent \paragraph{\emph{\textbf{$L_c$ and $L_{KL}$}}} For the ablation into clustering losses, we found that removing KL Loss (using only $L_c$) drops performance to 24.24\%, removing clustering loss (using only $L_{KL}$) drops to 23.32\%, while using both these losses gives 25.98\% for the case of N = 50 in \tabref{tab:main_results}.
We can conclude that both the clustering loss as well as the KL divergence loss are necessary as they offer complementary benefits (discussed in Sec 3.3).

% \subsection{Number of clusters}
% \label{subsec:experiment_on_clusters}

\vspace{-1em}
\noindent \paragraph{\emph{\textbf{Number of clusters}}} An important aspect of our formulation is the choice of number of clusters $K$ for the clustering approach in~\eqref{eq:clustering_loss}. From \figref{fig:clustering_exp}, K=10 clusters works well for the case of $N=50$. This concurs well with our intuition that a small value of $K$, like 5, would adversely affect the discriminative performance of the original task while a large value of $K$, like 20, would not encourage the semantic transfer we are after, as even related categories might form distinct clusters with no overlap 

% To provide more insight into the choice of $K$, we plot the effect of number of clusters on the segmentation performance in~\figref{fig:clustering_exp} for the setting of $\sigma=1\% (N=50)$. The number of distinct labels in GTA/Cityscapes is 19, while SUNRGB has 13 labels. For a very low value of $K$, the number of clusters would be very few which would adversely affect the discriminative performance of the original task and also result in many noisy alignments. Similarly, a large value of $K$ would not encourage the semantic transfer we are after, as even related categories might form distinct clusters with no overlap. From \figref{fig:clustering_exp}, we find that using $K=10$ clusters works best to balance this trade-off for our choice of datasets. 

% \subsection{Unsupervised Zero Shot Adaptation}

\vspace{-1em}
\paragraph{\emph{\textbf{Unsupervised Zero Shot Adaptation}}}

With a slight modification, our approach also works well for the problem of zero shot adaptation, when no (labeled, or unlabeled) examples are available from the target domain. 
% This setting is similar to the previously proposed RT-IRT based adaptation~\cite{wang2019conditional}, but in a more generalized framework with completely different tasks extended to semantic segmentation. 
For learning some task specific information, we assume availability of synthetically generated samples from the target domain. In our case, we render artificial indoor scenes from SceneNet~\cite{mccormac2017scenenet} dataset and use it in conjunction with our approach. We use this synthetically generated data from SceneNet instead of SUNRGB in the formulation, in \eqref{eq:supervised_loss} and \eqref{eq:clustering_loss} instead of $\D_t$. 

We compare our approach against the baselines where we use a classifier trained on SceneNet directly on SUNRGB. We report the results in \tabref{tab:zero_shot}, and our method which jointly optimizes a clustering objective along with an adversarial objective performs much better than the baselines that use only synthetic images from SceneNet. We believe that is due to the complementary knowledge that the network is able to infer through our approach.
% by learning the discriminative features from the SceneNet dataset, and more abstract lower level representations from GTA, resulting in superior performance without even using any real images from the target domain. 
Our method even improves upon plain joint training on labeled GTA and SceneNet datasets from $\sim17\%$ to $\sim22.8\%$, indicating that the benefit is not only due to increase in labeled data, but due to alignment as well.
% To verify the the fact that the benefit is not only due to the increase in amounts of labeled data, we also compare our approach against joint training the model on labeled GTA and SceneNet datasets, and report considerable absolute improvement  using $K=20$ clusters. 
Additionally, a network which learns without any real data from target domain should ideally generalize well to any similar datasets. Indeed, we observe from \tabref{tab:zero_shot} that the improvement on performance is not restricted to SUNRGB alone, but also observed on NYUv2~\cite{silberman2012indoor} validation set across all the baselines. 

% \subsection{Label Distribution}

% For training the model using the proposed approach, we require $N$ labeled examples from the target SUN-RGB dataset. 
% % In all our experiments, we choose the first $N$ examples from the official training set as the labeled target dataset $\D_t^l$. 
% Since no official split is available for a few shot setting like ours, we randomly choose a subset of train examples as the few shot examples $\D_t^l$ and fix this set over all the ablation studies. Through \figref{fig:robust_exp}, we demonstrate that our clustering based approach is robust towards the particular subset used, and the method outperforms the baselines as well as the adversarial approach irrespective of the subset used. However, the values vary over a wide range due to the disparity in the particular images used, which underlines the importance of establishing a standard few shot learning benchmark datasets for semantic segmentation as a future work.
% We also show the label distribution in our setting compared to the global distribution from the complete train set in \figref{fig:label_dist} for $N=50$ and $N=200$. The percentage of pixels of each class remain the same even in our few shot settings, except for classes like \textit{train} and \textit{sofa}, which are very scarcely present.
% Similar to any semantic segmentation task, the label distribution is not uniform across all the classes in the images. We show the label distribution of the chosen samples in \figref{fig:label_distribution} for $N=50$ and $N=200$ when compared to the total label distribution.




==> eccv2020kit/scripts/rebuttal.tex <==
\paragraph{\textit{Importance of our adaptation setting}[R2,R4]} 

Firstly, we strongly believe that the community needs to move ahead from the established conventions in domain adaptation, such as purely covariate shift, to achieve practical benefits. In this regard, our work follows recent advances like universal adaptation, where we even relax the constraint that source and target domains have any overlap. Therefore, ours is the most general setting for domain adaptation so far in the literature, which we believe is challenging yet useful, and indeed needs to be studied to extract potential practical benefits.

Furthermore, our particular instantiation, which involves transfer from a synthetic outdoor dataset (like GTA) to a real indoor dataset (like SUNRGB), is indeed relevant. Indoor settings contain a rich variety of objects and scenes with a variety of material and lighting properties, and it takes significant cost and efforts to accurately create and maintain assets even for synthetic indoor datasets. We also note the paucity of more indoor scene datasets currently for this exact reason, and existing datasets like SceneNet~\cite{mccormac2017scenenet} suffer from limited diversity in generated scenes. 
%
For example, a recent indoor scene dataset OpenRooms~\cite{li2020openrooms} takes almost 30,000 GPU hours to create the dataset. Also note that our proposed approach is generic enough to be applied to other settings such as medical images and fine-grained wildlife recognition, but we restrict our focus to semantic segmentation datasets in this particular work. 


% \paragraph{Effect of the number of clusters K}

\paragraph{\textit{Role of auxiliary intermediate domain}[R1,R4]} 
%
The intuition behind using an intermediate domain is to ease the adaptation process between the synthetic source domain data and real target domain data, which differ in both the appearance and the label spaces (categories). 
The use of an unlabeled domain bridge leads to no degradation with respect to a direct GTA to SUN adaptation for N = 200 (33.5\% without and 33.4\% with), while leading to a noticeable benefit for N = 50 (25.0\% without and 26.0\% with bridge domain). We will include this comparison in the final version. 

\paragraph{\textit{Comparison with semi-supervised methods}[R2,R4]} We thank the reviewers for bringing this to our notice, we will add citations to these works in an updated version of the paper. We indeed conducted experiments comparing our method with semi-supervised methods, and include the results in \tabref{tab:semi}. For \cite{hung2018adversarial}, we use the unlabeled and labeled image sets from SUN-RGB to run the experiments. For \cite{kalluri2019universal}, we follow the setting of their paper and use $N$ labeled examples from source and target, and use the rest of images without annotations.

As shown in the table, our method performs much better compared to the semi-supervised learning algorithms for lesser amounts of supervision as the latter do not make use of supervision available in the source domain at all. We will add this comparison in the final version of the paper.  

\begin{table*}
  \centering
  \resizebox{0.6\textwidth}{!}{
\begin{tabular}{l c c c c}
\toprule
 Method & N=50 & N=200 & N=500 & N=1500 \\
\midrule
UnivSeg~\cite{kalluri2019universal} & 22.21  & 31.32 & 36.08 & 42.10 \\
AdvSemiSeg~\cite{hung2018adversarial} & 24.72 & 33.22 & 38.46 & 45.10 \\
C2A [Ours] & 25.98 & 33.37 & 37.41 & 43.16 \\

\midrule
\end{tabular}}
\vspace{1em}
\caption{Comparison of semi-supervised methods with C2A for various levels of supervision on target SunRGB dataset. Clearly, C2A gives better accuracy than other semi-supervised methods at lower supervisions, for example N=50.
}
  \label{tab:semi}
\end{table*}


\paragraph{\textit{Related Works}[R4]} 

We are happy to cite the mentioned works and thank the reviewer for bringing them to our notice. Note however that they are not closely related. To emphasize: prior works consider the classical setting of completely matching source and target domains (Tang et.al, Wu et.al and Toldo et.al.,) or partial overlap in open world setting (Gong et.al), using clustering as a means to achieve one-to-one alignment between source and target. In contrast, we use clustering to selectively align source and target across disjoint label spaces. Similarly, our zero-hot adaptation setting is uniquely poised to achieve transfer between datasets with completely disjoint label spaces. 

\paragraph{}
